Language-Specific Effects of Tokenizer Choice in Multilingual Language Models

Tokenizer choice affects multilingual language modeling, but vocabulary capacity is finite and vocabulary size is often constrained: improving representation for some languages often comes at the expense of others. We therefore ask whether tokenizer choice matters equally across languages, a question that the current literature leave unanswered. To this end, we train 123 language models spanning 54 tokenizers. In the main comparison, architecture, training corpus, training-token budget, and optimization are held fixed, so the models differ only in their tokenizer. We find that tokenizer choice matters more for languages with less language-model training data: across the 54 tokenizers, the standard deviation of a language's bits-per-byte (BPB) increases as its model training-data share decreases (Spearman rho = -0.52 over the 31 trained languages and -0.69 over the 28 written with word boundaries). Leaving a language out of tokenizer training raises its BPB in every language we study, and the penalty tends to be larger for languages with less language-model training data. Giving lower-resource languages a larger share of tokenizer-training data, however, does not unconditionally help those languages: both equal weighting and an allocation inverting the shares with respect to the language model training data increase their BPB, particularly when language-model training repeats data. Finally, which intrinsic tokenizer properties are associated with better BPB differs across languages, providing further evidence that what makes a good tokenizer depends on the language. We find that the metrics quantifying these properties can be successfully used to predict downstream models' pairwise BPB rankings, suggesting a practical strategy for screening tokenizer candidates before training language models.

==> crosslingual_tables/equalweight.tex <==
\begin{tabular}{lccc}
\toprule
\textbf{Variant (vs.\ balanced baseline)} & $\Delta$ \textbf{mean} & $\Delta$ \textbf{tail} & \textbf{Spearman} $\rho$ \\
\midrule
Equal weights (GPT-4o)             & \rrev{$+0.0107$} & \rrev{$+0.0177$} & $\mathbf{-0.61}^{*}$ \\
% prov: results/correlations/equal_weighting_postboundary.json#results["nominal sampling weight"][contrast=full-128k-allmulti-equal-bpe].{mean_delta,tail_mean_delta}
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-allmulti-equal-bpe].spearman_rho (Spearman column on the realized byte share, ruling 2026-09-23)
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-allmulti-equal-bpe].spearman_p (supports the star, not printed)
Equal weights (Claude)             & \rrev{$+0.0064$} & \rrev{$+0.0162$} & \rrev{$\mathbf{-0.52}^{*}$} \\
% prov: results/correlations/equal_weighting_postboundary.json#results["nominal sampling weight"][contrast=full-128k-claude-allmulti-equal-bpe].{mean_delta,tail_mean_delta}
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-claude-allmulti-equal-bpe].spearman_rho (Spearman column on the realized byte share, ruling 2026-09-23)
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-claude-allmulti-equal-bpe].spearman_p (supports the star, not printed)
Equal weights (Punct)              & \rrev{$+0.0015$} & \rrev{$+0.0031$} & \rrev{$-0.07$} \\
% prov: results/correlations/equal_weighting_postboundary.json#results["nominal sampling weight"][contrast=full-128k-punct-allmulti-equal-bpe].{mean_delta,tail_mean_delta}
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-punct-allmulti-equal-bpe].spearman_rho (Spearman column on the realized byte share, ruling 2026-09-23)
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-punct-allmulti-equal-bpe].spearman_p (supports the star, not printed)
Equal weights (GPT-4o, NFC)        & \rrev{$+0.0054$} & \rrev{$+0.0099$} & \rrev{$-0.34$} \\
% prov: results/correlations/equal_weighting_postboundary.json#results["nominal sampling weight"][contrast=full-128k-gpt4o-allmulti-equal-nfc-bpe].{mean_delta,tail_mean_delta}
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-gpt4o-allmulti-equal-nfc-bpe].spearman_rho (Spearman column on the realized byte share, ruling 2026-09-23)
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-gpt4o-allmulti-equal-nfc-bpe].spearman_p (supports the star, not printed)
Equal weights, no repeat sampling  & \rrev{$+0.0060$} & \rrev{$+0.0120$} & \rrev{$\mathbf{-0.44}^{*}$} \\
% prov: results/correlations/equal_weighting_postboundary.json#results["nominal sampling weight"][contrast=full-128k-gpt4o-allmulti-equal-norepeat-bpe].{mean_delta,tail_mean_delta}
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-gpt4o-allmulti-equal-norepeat-bpe].spearman_rho (Spearman column on the realized byte share, ruling 2026-09-23)
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-gpt4o-allmulti-equal-norepeat-bpe].spearman_p (supports the star, not printed)
\midrule
File cap only (control)            & \rrev{$-0.0035$} & \rrev{$-0.0039$} & \rrev{$+0.17$} \\
% prov: results/correlations/equal_weighting_postboundary.json#results["nominal sampling weight"][contrast=full-128k-gpt4o-balanced-maxfiles50-bpe].{mean_delta,tail_mean_delta}
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-gpt4o-balanced-maxfiles50-bpe].spearman_rho (Spearman column on the realized byte share, ruling 2026-09-23)
% prov: results/correlations/equal_weighting_postboundary.json#results["realized mixture byte share"][contrast=full-128k-gpt4o-balanced-maxfiles50-bpe].spearman_p (supports the star, not printed)
\bottomrule
\end{tabular}


==> crosslingual_tables/exclusion-general-difference.tex <==
\begin{tabular}{p{0.34\linewidth}rrrr}
\toprule
\textbf{\# of coverage tokenizers that exclude the language} &\shortstack[r]{\textbf{\# of languages }\\\textbf{in group}}  & \shortstack[r]{\textbf{Difference in}\\\textbf{31-language mean}} & \shortstack[r]{\textbf{Mean}\\\textbf{penalty}} & \textbf{Ratio} \\
\midrule
One (English-only) & 5 & \rrev{$0.0278$} & \rrev{$0.0671$} & $0.41$ \\
% prov: results/correlations/crosslingual_v2/coverage_exclusion.json#general_rise_by_stratum.excluded_by_1_english.{general_rise_of_tokenizer_means,mean_penalty,general_rise_share_of_mean_penalty}
% prov: results/correlations/crosslingual_v2/coverage_exclusion.json#general_rise_by_stratum.excluded_by_1_english.n_languages (printed as a rounded integer, not printed as a decimal)
Two (English-only, high-resource) & 15 & \rrev{$0.0233$} & $0.0213$ & \rrev{$1.09$} \\
% prov: results/correlations/crosslingual_v2/coverage_exclusion.json#general_rise_by_stratum.excluded_by_2.{general_rise_of_tokenizer_means,mean_penalty,general_rise_share_of_mean_penalty}
% prov: results/correlations/crosslingual_v2/coverage_exclusion.json#general_rise_by_stratum.excluded_by_2.n_languages (printed as a rounded integer, not printed as a decimal)
Three (English-only, high-resource, high-and-mid-resource) & 10 & \rrev{$0.0236$} & \rrev{$0.0330$} & \rrev{$0.72$} \\
% prov: results/correlations/crosslingual_v2/coverage_exclusion.json#general_rise_by_stratum.excluded_by_3.{general_rise_of_tokenizer_means,mean_penalty,general_rise_share_of_mean_penalty}
% prov: results/correlations/crosslingual_v2/coverage_exclusion.json#general_rise_by_stratum.excluded_by_3.n_languages (printed as a rounded integer, not printed as a decimal)
\bottomrule
\end{tabular}



==> crosslingual_tables/full-flores.tex <==
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{\textbf{Agg.\ $\rho$}} & \multicolumn{2}{c}{\textbf{Median lang.\ $\rho$}} & \multicolumn{2}{c}{\textbf{Sig.}} \\
\textbf{Intrinsic metric} & \textbf{tr.-31} & \textbf{all-214} & \textbf{trained} & \textbf{untrained} & \textbf{tr.} & \textbf{untr.} \\
\midrule
R\'enyi eff.\ ($\alpha{=}2$) & \rrev{$-0.455$} & \rrev{$-0.193$} & \rrev{$-0.288$} & \rrev{$-0.072$} & \rrev{9} & \rrev{11} \\ 
% prov: results/correlations/crosslingual_v2/full_flores_decomposition.json#per_metric.renyi_2.0
Trigram entropy              & \rrev{$-0.446$} & \rrev{$+0.130$} & \rrev{$-0.328$} & \rrev{$+0.080$} & \rrev{15} & \rrev{34} \\ 
% prov: results/correlations/crosslingual_v2/full_flores_decomposition.json#per_metric.trigram_entropy
Compression rate             & \rrev{$-0.326$} & \rrev{$+0.227$} & \rrev{$-0.226$} & \rrev{$+0.106$} & \rrev{9} & \rrev{56} \\ 
% prov: results/correlations/crosslingual_v2/full_flores_decomposition.json#per_metric.compression_rate
UTF-8 char split             & \rrev{$+0.331$} & \rrev{$-0.194$} & \rrev{$+0.348$} & \rrev{$-0.047$} & \rrev{17} & \rrev{34} \\ 
% prov: results/correlations/crosslingual_v2/full_flores_decomposition.json#per_metric.utf8_char_split
Bigram entropy               & \rrev{$-0.286$} & $+0.052$ & \rrev{$-0.214$} & \rrev{$+0.024$} & \rrev{6} & \rrev{40} \\ 
% prov: results/correlations/crosslingual_v2/full_flores_decomposition.json#per_metric.bigram_entropy
Unigram entropy              & \rrev{$-0.274$} & \rrev{$+0.100$} & \rrev{$-0.224$} & \rrev{$+0.068$} & \rrev{5} & \rrev{50} \\ 
% prov: results/correlations/crosslingual_v2/full_flores_decomposition.json#per_metric.unigram_entropy
UTF-8 boundary crossing      & \rrev{$+0.266$} & \rrev{$-0.126$} & \rrev{$+0.273$} & \rrev{$0.005$} & \rrev{5} & \rrev{10} \\ 
% prov: results/correlations/crosslingual_v2/full_flores_decomposition.json#per_metric.utf8_boundary_crossing
Vocab utilization            & \rrev{$-0.040$} & \rrev{$+0.245$} & \rrev{$-0.104$} & \rrev{$+0.079$} & \rrev{2} & \rrev{33} \\ 
% prov: results/correlations/crosslingual_v2/full_flores_decomposition.json#per_metric.vocab_utilization
Fertility                    & \rrev{$+0.033$} & \rrev{$-0.303$} & \rrev{$+0.008$} & \rrev{$-0.125$} &  1 & \rrev{28} \\ 
% prov: results/correlations/crosslingual_v2/full_flores_decomposition.json#per_metric.fertility
\bottomrule
\end{tabular}


==> crosslingual_tables/grid.tex <==
\adjustbox{max width=\textwidth}{%
\begin{tabular}{lllllrc}
\toprule
\textbf{Tokenizer} & \textbf{Algorithm} & \textbf{Pretok} & \textbf{Data} & \textbf{Norm.} & \textbf{Vocab} & \textbf{Family} \\
\midrule
BPE GPT-4o (balanced)            & BPE & GPT-4o      & balanced          & --- & $128{,}256$ & G \\
% prov: results/correlations/crosslingual_v2/families.csv#gpt4o-balanced-bpe; tier1_vocab_census.json#vocab_sizes.gpt4o-balanced-bpe
BPE GPT-4o (balanced, file cap)  & BPE & GPT-4o      & balanced          & --- & $128{,}256$ & G \\
% prov: results/correlations/crosslingual_v2/families.csv#gpt4o-balanced-maxfiles50-bpe; tier1_vocab_census.json#vocab_sizes.gpt4o-balanced-maxfiles50-bpe
BPE GPT-4o NFC (balanced)        & BPE & GPT-4o      & balanced          & NFC & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#gpt4o-balanced-nfc-bpe; tier1_vocab_census.json#vocab_sizes.gpt4o-balanced-nfc-bpe
BPE GPT-4o (english)$^{a}$       & BPE & GPT-4o      & english           & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#gpt4o-english-fullbyte-bpe; tier1_vocab_census.json#vocab_sizes.gpt4o-english-fullbyte-bpe
BPE GPT-4o (code)                & BPE & GPT-4o      & code              & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#gpt4o-code-bpe; tier1_vocab_census.json#vocab_sizes.gpt4o-code-bpe
BPE GPT-4o (highres)             & BPE & GPT-4o      & highres           & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#highres-bpe; tier1_vocab_census.json#vocab_sizes.highres-bpe
BPE GPT-4o (highmid)             & BPE & GPT-4o      & highmid           & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#highmid-bpe; tier1_vocab_census.json#vocab_sizes.highmid-bpe
BPE GPT-4o (all-equal)           & BPE & GPT-4o      & all-equal         & --- & $128{,}256$ & fam05 \\
% prov: results/correlations/crosslingual_v2/families.csv#allmulti-equal-bpe; tier1_vocab_census.json#vocab_sizes.allmulti-equal-bpe
BPE GPT-4o (all-equal, no repeat)& BPE & GPT-4o      & all-equal         & --- & $128{,}256$ & fam05 \\
% prov: results/correlations/crosslingual_v2/families.csv#gpt4o-allmulti-equal-norepeat-bpe; tier1_vocab_census.json#vocab_sizes.gpt4o-allmulti-equal-norepeat-bpe
BPE GPT-4o NFC (all-equal)       & BPE & GPT-4o      & all-equal         & NFC & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#gpt4o-allmulti-equal-nfc-bpe; tier1_vocab_census.json#vocab_sizes.gpt4o-allmulti-equal-nfc-bpe
BPE GPT-4o NFC (fw2full)         & BPE & GPT-4o      & fw2full           & NFC & $128{,}000$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#bpe-nfc-gpt4-fineweb2full; tier1_vocab_census.json#vocab_sizes.bpe-nfc-gpt4-fineweb2full
BPE GPT-4o script-enc.\ (bal.)$^{s}$ & BPE & GPT-4o  & balanced          & NFC & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#scripttok-bpe-scriptenc_gpt4o_cb; tier1_vocab_census.json#vocab_sizes.scripttok-bpe-scriptenc_gpt4o_cb
BPE Claude (balanced)            & BPE & Claude      & balanced          & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#claude-balanced-bpe; tier1_vocab_census.json#vocab_sizes.claude-balanced-bpe
BPE Claude NFC (balanced)        & BPE & Claude      & balanced          & NFC & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#claude-balanced-nfc-bpe; tier1_vocab_census.json#vocab_sizes.claude-balanced-nfc-bpe
BPE Claude (english)$^{b}$       & BPE & Claude      & english           & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#claude-english-bpe; tier1_vocab_census.json#vocab_sizes.claude-english-bpe
BPE Claude (all-equal)           & BPE & Claude      & all-equal         & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#claude-allmulti-equal-bpe; tier1_vocab_census.json#vocab_sizes.claude-allmulti-equal-bpe
BPE Claude V2 (balanced)         & BPE & Claude V2   & balanced          & NFD$^{d}$ & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#clauderev-balanced-bpe; tier1_vocab_census.json#vocab_sizes.clauderev-balanced-bpe
BPE GPT-2 (balanced)             & BPE & GPT-2       & balanced          & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#gpt2-balanced-bpe; tier1_vocab_census.json#vocab_sizes.gpt2-balanced-bpe
BPE Punct (balanced)             & BPE & Punct       & balanced          & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#punct-balanced-bpe; tier1_vocab_census.json#vocab_sizes.punct-balanced-bpe
BPE Punct (english)$^{b}$        & BPE & Punct       & english           & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#punct-english-bpe; tier1_vocab_census.json#vocab_sizes.punct-english-bpe
BPE Punct (all-equal)            & BPE & Punct       & all-equal         & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#punct-allmulti-equal-bpe; tier1_vocab_census.json#vocab_sizes.punct-allmulti-equal-bpe
BPE RightAlign (balanced)        & BPE & RightAlign  & balanced          & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#rightalign-balanced-bpe; tier1_vocab_census.json#vocab_sizes.rightalign-balanced-bpe
BPE RightAlign NFC (balanced)    & BPE & RightAlign  & balanced          & NFC & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#rightalign-balanced-nfc-bpe; tier1_vocab_census.json#vocab_sizes.rightalign-balanced-nfc-bpe
BPE Whitespace (balanced)        & BPE & Whitespace  & balanced          & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#whitespace-balanced-bpe; tier1_vocab_census.json#vocab_sizes.whitespace-balanced-bpe
BPE Whitespace (multi-heavy)     & BPE & Whitespace  & multi-heavy       & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#whitespace-multiheavy-bpe; tier1_vocab_census.json#vocab_sizes.whitespace-multiheavy-bpe
BPE Clean NFC (balanced)         & BPE & Clean       & balanced          & NFC & $128{,}004$ & fam00 \\
% prov: results/correlations/crosslingual_v2/families.csv#bpe-nfc-clean-balanced; tier1_vocab_census.json#vocab_sizes.bpe-nfc-clean-balanced
BPE Clean no-mark NFC (bal.)     & BPE & Clean no-mark & balanced        & NFC & $128{,}000$ & fam00 \\
% prov: results/correlations/crosslingual_v2/families.csv#bpe-nfc-clean-nomark-balanced; tier1_vocab_census.json#vocab_sizes.bpe-nfc-clean-nomark-balanced
BPE Clean plus2 NFC (bal.)       & BPE & Clean plus2 & balanced          & NFC & $128{,}256$ & fam00 \\
% prov: results/correlations/crosslingual_v2/families.csv#bpe-nfc-plus2-balanced; tier1_vocab_census.json#vocab_sizes.bpe-nfc-plus2-balanced
BPE Clean plus3 NFC (bal.)       & BPE & Clean plus3 & balanced          & NFC & $128{,}256$ & fam00 \\
% prov: results/correlations/crosslingual_v2/families.csv#bpe-nfc-plus3-balanced; tier1_vocab_census.json#vocab_sizes.bpe-nfc-plus3-balanced
BPE Clean NFC (fw2full)          & BPE & Clean       & fw2full           & NFC & $128{,}000$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#bpe-nfc-clean-fineweb2full; tier1_vocab_census.json#vocab_sizes.bpe-nfc-clean-fineweb2full
Mistral-Nemo                     & BPE & Mistral-Nemo & off-the-shelf    & --- & $131{,}072$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#apertus; tier1_vocab_census.json#vocab_sizes.apertus
LLaMA-3                          & BPE & LLaMA-3     & off-the-shelf     & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#llama3; tier1_vocab_census.json#vocab_sizes.llama3
\midrule
Unigram GPT-4o (balanced)        & UnigramLM & GPT-4o     & balanced     & --- & $128{,}256$ & D \\
% prov: results/correlations/crosslingual_v2/families.csv#gpt4o-balanced-unigram; tier1_vocab_census.json#vocab_sizes.gpt4o-balanced-unigram
Unigram GPT-4o tuned (balanced)  & UnigramLM & GPT-4o     & balanced     & --- & $128{,}256$ & D \\
% prov: results/correlations/crosslingual_v2/families.csv#gpt4o-balanced-unigram-tuned; tier1_vocab_census.json#vocab_sizes.gpt4o-balanced-unigram-tuned
Unigram GPT-4o (highres)         & UnigramLM & GPT-4o     & highres      & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#highres-unigram; tier1_vocab_census.json#vocab_sizes.highres-unigram
Unigram GPT-4o (highmid)         & UnigramLM & GPT-4o     & highmid      & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#highmid-unigram; tier1_vocab_census.json#vocab_sizes.highmid-unigram
Unigram Claude (balanced)        & UnigramLM & Claude     & balanced     & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#claude-balanced-unigram; tier1_vocab_census.json#vocab_sizes.claude-balanced-unigram
Unigram RightAlign (balanced)    & UnigramLM & RightAlign & balanced     & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#rightalign-balanced-unigram; tier1_vocab_census.json#vocab_sizes.rightalign-balanced-unigram
Unigram Whitespace (balanced)$^{c}$ & UnigramLM & Whitespace & balanced  & --- & $128{,}256$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#whitespace-balanced-unigram; tier1_vocab_census.json#vocab_sizes.whitespace-balanced-unigram
\midrule
MinGram script-enc.\ (balanced)$^{s}$ & MinGram & SCRIPT   & balanced    & NFC & $128{,}256$ & fam06 \\
% prov: results/correlations/crosslingual_v2/families.csv#scripttok-mingram-scriptenc_cb; tier1_vocab_census.json#vocab_sizes.scripttok-mingram-scriptenc_cb
MinGram script-enc., split newlines$^{s}$ & MinGram & SCRIPT & balanced  & NFC & $128{,}256$ & fam06 \\
% prov: results/correlations/crosslingual_v2/families.csv#scripttok-mingram-scriptenc_cb_nl; tier1_vocab_census.json#vocab_sizes.scripttok-mingram-scriptenc_cb_nl
\midrule
SuperBPE GPT-4o (balanced)       & SuperBPE & GPT-4o      & balanced     & --- & $128{,}004$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#superbpe-gpt4o-balanced; tier1_vocab_census.json#vocab_sizes.superbpe-gpt4o-balanced
SuperBPE Clean C2 (balanced)     & SuperBPE & Clean       & balanced     & NFC & $128{,}004$ & C \\
% prov: results/correlations/crosslingual_v2/families.csv#superbpe-clean-c2-balanced; tier1_vocab_census.json#vocab_sizes.superbpe-clean-c2-balanced
SuperBPE Clean C3 (balanced)     & SuperBPE & Clean       & balanced     & NFC & $128{,}004$ & C \\
% prov: results/correlations/crosslingual_v2/families.csv#superbpe-clean-c3-balanced; tier1_vocab_census.json#vocab_sizes.superbpe-clean-c3-balanced
SuperBPE Punct t64k (bal.-half)  & SuperBPE & Punct       & balanced-half & --- & $128{,}004$ &  \\
% prov: results/correlations/crosslingual_v2/families.csv#punct-balancedhalf-superbpe-t64k-copy; tier1_vocab_census.json#vocab_sizes.punct-balancedhalf-superbpe-t64k-copy
SuperBPE/PA-BPE GPT-4o (balanced) & SuperBPE/PA-BPE & GPT-4o & balanced    & NFC & $128{,}004$ & B \\
% prov: results/correlations/crosslingual_v2/families.csv#superbpe-pabpe-nfc-gpt4-balanced; tier1_vocab_census.json#vocab_sizes.superbpe-pabpe-nfc-gpt4-balanced
SuperBPE/PA-BPE GPT-4o t64k       & SuperBPE/PA-BPE & GPT-4o & balanced    & NFC & $128{,}004$ & B \\
% prov: results/correlations/crosslingual_v2/families.csv#superbpe-pabpe-nfc-gpt4-t64k; tier1_vocab_census.json#vocab_sizes.superbpe-pabpe-nfc-gpt4-t64k
\midrule
PA-BPE GPT-4o (balanced)          & PA-BPE & GPT-4o       & balanced       & NFC & $127{,}826$ & A \\
% prov: results/correlations/crosslingual_v2/families.csv#pabpe-nfc-gpt4-balanced; tier1_vocab_census.json#vocab_sizes.pabpe-nfc-gpt4-balanced
PA-BPE GPT-4o hybrid-window (bal.)& PA-BPE & GPT-4o       & balanced       & NFC & $127{,}826$ & A \\
% prov: results/correlations/crosslingual_v2/families.csv#pabpe-nfc-gpt4-balanced-hybridwindow; tier1_vocab_census.json#vocab_sizes.pabpe-nfc-gpt4-balanced-hybridwindow
PA-BPE Clean (balanced)          & PA-BPE & Clean       & balanced       & NFC & $127{,}836$ &   \\
% prov: results/correlations/crosslingual_v2/families.csv#pabpe-nfc-clean-balanced; tier1_vocab_census.json#vocab_sizes.pabpe-nfc-clean-balanced
PA-BPE GPT-4o (fw2full)           & PA-BPE & GPT-4o       & fw2full        & NFC & $127{,}825$ & E \\
% prov: results/correlations/crosslingual_v2/families.csv#pabpe-nfc-gpt4-fineweb2full; tier1_vocab_census.json#vocab_sizes.pabpe-nfc-gpt4-fineweb2full
PA-BPE GPT-4o hybrid-win.\ (fw2full) & PA-BPE & GPT-4o    & fw2full        & NFC & $127{,}825$ & E \\
% prov: results/correlations/crosslingual_v2/families.csv#pabpe-nfc-gpt4-fineweb2full-hybridwindow; tier1_vocab_census.json#vocab_sizes.pabpe-nfc-gpt4-fineweb2full-hybridwindow
PA-BPE Clean (fw2full)           & PA-BPE & Clean       & fw2full        & NFC & $127{,}835$ & F \\
% prov: results/correlations/crosslingual_v2/families.csv#pabpe-nfc-clean-fineweb2full; tier1_vocab_census.json#vocab_sizes.pabpe-nfc-clean-fineweb2full
PA-BPE Clean hybrid-win.\ (fw2full) & PA-BPE & Clean    & fw2full        & NFC & $127{,}835$ & F \\
% prov: results/correlations/crosslingual_v2/families.csv#pabpe-nfc-clean-fineweb2full-hybridwindow; tier1_vocab_census.json#vocab_sizes.pabpe-nfc-clean-fineweb2full-hybridwindow
\bottomrule
\end{tabular}}


==> crosslingual_tables/inversion-multiblimp.tex <==
\begin{tabular}{lccc}
\toprule
\textbf{Variant} & \textbf{Mean $\Delta$acc.} & \textbf{Spearman} $\rho$ & $p$ \\
\midrule
L2 (inverted)    & $-0.0054$ & \rrev{$+0.313$} & \rrev{$0.136$} \\
% prov: results/correlations/resource_inversion.json#multiblimp_secondary.per_arm.L2.{mean_dacc,spearman_rho_dacc_vs_log_lm_weight,p}
P1 (permuted)    & $-0.0085$ & \rrev{$+0.292$} & \rrev{$0.166$} \\
% prov: results/correlations/resource_inversion.json#multiblimp_secondary.per_arm.P1.{mean_dacc,spearman_rho_dacc_vs_log_lm_weight,p}
P2 (permuted)    & $-0.0071$ & \rrev{$+0.227$} & \rrev{$0.286$} \\
% prov: results/correlations/resource_inversion.json#multiblimp_secondary.per_arm.P2.{mean_dacc,spearman_rho_dacc_vs_log_lm_weight,p}
E1 (no English)  & $-0.0050$ & \rrev{$+0.208$} & \rrev{$0.330$} \\
% prov: results/correlations/resource_inversion.json#multiblimp_secondary.per_arm.E1.{mean_dacc,spearman_rho_dacc_vs_log_lm_weight,p}
\bottomrule
\end{tabular}


==> crosslingual_tables/inversion-offset.tex <==
\begin{tabular}{lccc}
\toprule
\textbf{Token-budget treatment} & \textbf{Offset} & \textbf{Fert.\ ratio} & \textbf{Interaction} ($p$) \\
\midrule
Joint fit (token-share covariate) & ---        & ---      & \rrev{$+0.0426$ ($1.3\times10^{-3}$)} \\ 
% prov: results/correlations/resource_inversion.json#fit.{interaction_coef,interaction_p}
Offset zero                       & $0$        & \rrev{$-0.102$} & \rrev{$+0.040$ ($2.9\times10^{-3}$)} \\ 
% prov: results/correlations/resource_inversion.json#offset_sensitivity.none_0.{dose_coef,interaction_coef,interaction_p}
Offset at the pooled point estimate & $-0.0128$  & \rrev{$-0.089$} & \rrev{$+0.040$ ($2.9\times10^{-3}$)} \\ 
% prov: results/correlations/resource_inversion.json#offset_sensitivity.g2_point.{beta_offset,dose_coef,interaction_coef,interaction_p}
Offset at the band's low end      & $-0.0429$  & \rrev{$-0.059$} & \rrev{$+0.040$ ($2.9\times10^{-3}$)} \\ 
% prov: results/correlations/resource_inversion.json#offset_sensitivity.g2_ci_low.{beta_offset,dose_coef,interaction_coef,interaction_p}
Offset at the band's high end     & $+0.0173$  & \rrev{$-0.119$} & \rrev{$+0.040$ ($2.9\times10^{-3}$)} \\ 
% prov: results/correlations/resource_inversion.json#offset_sensitivity.g2_ci_high.{beta_offset,dose_coef,interaction_coef,interaction_p}
\bottomrule
\end{tabular}


==> crosslingual_tables/inversion-xcopa.tex <==
\begin{tabular}{lccc}
\toprule
\textbf{Variant} & \textbf{Mean $\Delta$acc.} & \textbf{Spearman} $\rho$ & $p$ \\
\midrule
L2 (inverted)    & $-0.0057$ & $-0.321$ & $0.482$ \\
% prov: results/correlations/crosslingual_v2/xcopa_battery.json#inversion_readout.per_arm.L2.{mean_dacc,spearman_rho_dacc_vs_log_lm_weight,p}
P1 (permuted)    & $-0.0009$ & \rrev{$-0.143$} & \rrev{$0.760$} \\
% prov: results/correlations/crosslingual_v2/xcopa_battery.json#inversion_readout.per_arm.P1.{mean_dacc,spearman_rho_dacc_vs_log_lm_weight,p}
P2 (permuted)    & $-0.0086$ & \rrev{$-0.464$} & \rrev{$0.294$} \\
% prov: results/correlations/crosslingual_v2/xcopa_battery.json#inversion_readout.per_arm.P2.{mean_dacc,spearman_rho_dacc_vs_log_lm_weight,p}
E1 (no English)  & $-0.0071$ & \rrev{$-0.714$} & \rrev{$0.071$} \\
% prov: results/correlations/crosslingual_v2/xcopa_battery.json#inversion_readout.per_arm.E1.{mean_dacc,spearman_rho_dacc_vs_log_lm_weight,p}
\bottomrule
\end{tabular}


==> crosslingual_tables/lang.tex <==
\adjustbox{max width=\textwidth}{%
\begin{tabular}{lllrrr@{\hspace{1.6em}}lllrrr}
\toprule
\textbf{Language} & \textbf{Code} & \textbf{Script} & \textbf{GB} & \textbf{\%} & \textbf{w} &
\textbf{Language} & \textbf{Code} & \textbf{Script} & \textbf{GB} & \textbf{\%} & \textbf{w} \\
\midrule
Russian    & \texttt{rus\_Cyrl} & Cyrillic & 4.521 & 18.1 & 0.1064 & Hungarian  & \texttt{hun\_Latn} & Latin    & 0.099 & 0.4 & 0.0051 \\
Spanish    & \texttt{spa\_Latn} & Latin    & 0.423 & 1.7 & 0.0245 & Vietnamese & \texttt{vie\_Latn} & Latin    & 0.109 & 0.4 & 0.0043 \\
German     & \texttt{deu\_Latn} & Latin    & 0.353 & 1.4 & 0.0238 & Czech      & \texttt{ces\_Latn} & Latin    & 0.077 & 0.3 & 0.0043 \\
French     & \texttt{fra\_Latn} & Latin    & 0.364 & 1.5 & 0.0206 & Greek      & \texttt{ell\_Grek} & Greek    & 0.108 & 0.4 & 0.0035 \\
Chinese    & \texttt{cmn\_Hani} & CJK      & 0.326 & 1.3 & 0.0191 & Thai       & \texttt{tha\_Thai} & Thai     & 0.087 & 0.3 & 0.0023 \\
Japanese   & \texttt{jpn\_Jpan} & CJK      & 0.204 & 0.8 & 0.0127 & Finnish    & \texttt{fin\_Latn} & Latin    & 0.034 & 0.1 & 0.0023 \\
Italian    & \texttt{ita\_Latn} & Latin    & 0.165 & 0.7 & 0.0119 & Slovak     & \texttt{slk\_Latn} & Latin    & 0.028 & 0.1 & 0.0020 \\
Portuguese & \texttt{por\_Latn} & Latin    & 0.189 & 0.8 & 0.0119 & Bulgarian  & \texttt{bul\_Cyrl} & Cyrillic & 0.052 & 0.2 & 0.0019 \\
Turkish    & \texttt{tur\_Latn} & Latin    & 0.152 & 0.6 & 0.0094 & Korean     & \texttt{kor\_Hang} & Hangul   & 0.029 & 0.1 & 0.0016 \\
Indonesian & \texttt{ind\_Latn} & Latin    & 0.236 & 0.9 & 0.0091 & Croatian   & \texttt{hrv\_Latn} & Latin    & 0.026 & 0.1 & 0.0017 \\
Polish     & \texttt{pol\_Latn} & Latin    & 0.107 & 0.4 & 0.0088 & Catalan    & \texttt{cat\_Latn} & Latin    & 0.014 & 0.1 & 0.0010 \\
Ukrainian  & \texttt{ukr\_Cyrl} & Cyrillic & 0.211 & 0.8 & 0.0068 & Hindi      & \texttt{hin\_Deva} & Devanagari & 0.032 & 0.1 & 0.0010 \\
Dutch      & \texttt{nld\_Latn} & Latin    & 0.071 & 0.3 & 0.0065 & Hebrew     & \texttt{heb\_Hebr} & Hebrew   & 0.025 & 0.1 & 0.0009 \\
Romanian   & \texttt{ron\_Latn} & Latin    & 0.097 & 0.4 & 0.0058 & Bengali    & \texttt{ben\_Beng} & Bengali  & 0.024 & 0.1 & 0.0007 \\
Arabic     & \texttt{arb\_Arab} & Arabic   & 0.168 & 0.7 & 0.0054 & Tamil      & \texttt{tam\_Taml} & Tamil    & 0.017 & 0.1 & 0.0004 \\
\bottomrule
\end{tabular}}


==> crosslingual_tables/magnitude.tex <==
\begin{tabular}{lrrrcrrrc}
\toprule
& \multicolumn{4}{c}{\textbf{FLORES+ BPB}} & \multicolumn{4}{c}{\textbf{MultiBLiMP accuracy}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
\textbf{Language} & spread & seed SD & ratio & clears & spread & seed SD & ratio & clears \\
\midrule
eng\_Latn & \rrev{\brev{0.0112}} & \rrev{\brev{0.0010}} & \rrev{\brev{11.00}} & yes & 0.0050 & \brev{0.0041} & \brev{1.20} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.eng_Latn.{flores,multiblimp}
rus\_Cyrl & \rrev{\brev{0.0040}} & \rrev{\brev{0.0011}} & \rrev{\brev{3.56}} & yes & 0.0035 & \brev{0.0018} & \brev{1.93} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.rus_Cyrl.{flores,multiblimp}
spa\_Latn & \rrev{\brev{0.0120}} & \rrev{\brev{0.0012}} & \rrev{\brev{10.17}} & yes & 0.0038 & \brev{0.0025} & \brev{1.54} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.spa_Latn.{flores,multiblimp}
deu\_Latn & \rrev{\brev{0.0084}} & \rrev{\brev{0.0016}} & \rrev{\brev{5.37}} & yes & 0.0038 & \brev{0.0010} & \brev{3.91} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.deu_Latn.{flores,multiblimp}
fra\_Latn & \rrev{\brev{0.0114}} & \rrev{\brev{0.0015}} & \rrev{\brev{7.39}} & yes & 0.0036 & \brev{0.0026} & \brev{1.40} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.fra_Latn.{flores,multiblimp}
cmn\_Hans & \rrev{\brev{0.0623}} & \rrev{\brev{0.0027}} & \rrev{\brev{23.43}} & yes & -- & -- & -- & -- \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.cmn_Hans.flores
jpn\_Jpan & \rrev{\brev{0.0249}} & \rrev{\brev{0.0013}} & \rrev{\brev{19.92}} & yes & -- & -- & -- & -- \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.jpn_Jpan.flores
ita\_Latn & \rrev{\brev{0.0123}} & \rrev{\brev{0.0019}} & \rrev{\brev{6.55}} & yes & 0.0062 & \brev{0.0040} & \brev{1.56} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.ita_Latn.{flores,multiblimp}
por\_Latn & \rrev{\brev{0.0113}} & \rrev{\brev{0.0010}} & \rrev{\brev{11.19}} & yes & 0.0050 & \brev{0.0022} & \brev{2.26} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.por_Latn.{flores,multiblimp}
tur\_Latn & \rrev{\brev{0.0111}} & \rrev{\brev{0.0020}} & \rrev{\brev{5.63}} & yes & 0.0104 & \brev{0.0109} & \brev{0.95} & \brev{no} \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.tur_Latn.{flores,multiblimp}
ind\_Latn & \rrev{\brev{0.0089}} & \rrev{\brev{0.0018}} & \rrev{\brev{5.07}} & yes & -- & -- & -- & -- \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.ind_Latn.flores
pol\_Latn & \rrev{\brev{0.0124}} & \rrev{\brev{0.0025}} & \rrev{\brev{4.98}} & yes & 0.0062 & \brev{0.0042} & \brev{1.47} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.pol_Latn.{flores,multiblimp}
ukr\_Cyrl & \rrev{\brev{0.0082}} & \rrev{\brev{0.0016}} & \rrev{\brev{5.04}} & yes & 0.0068 & \brev{0.0067} & \brev{1.02} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.ukr_Cyrl.{flores,multiblimp}
nld\_Latn & \rrev{\brev{0.0106}} & \rrev{\brev{0.0032}} & \rrev{\brev{3.35}} & yes & 0.0060 & \brev{0.0067} & \brev{0.90} & \brev{no} \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.nld_Latn.{flores,multiblimp}
ron\_Latn & \rrev{\brev{0.0097}} & \rrev{\brev{0.0021}} & \rrev{\brev{4.59}} & yes & 0.0065 & \brev{0.0029} & \brev{2.23} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.ron_Latn.{flores,multiblimp}
arb\_Arab & \rrev{\brev{0.0097}} & \rrev{\brev{0.0014}} & \rrev{\brev{7.17}} & yes & 0.0103 & \brev{0.0056} & \brev{1.83} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.arb_Arab.{flores,multiblimp}
hun\_Latn & \rrev{\brev{0.0141}} & \rrev{\brev{0.0022}} & \rrev{\brev{6.42}} & yes & 0.0079 & \brev{0.0074} & \brev{1.08} & \brev{yes} \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.hun_Latn.{flores,multiblimp}
vie\_Latn & \rrev{\brev{0.0212}} & \rrev{\brev{0.0015}} & \rrev{\brev{14.51}} & yes & -- & -- & -- & -- \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.vie_Latn.flores
ces\_Latn & \rrev{\brev{0.0116}} & \rrev{\brev{0.0018}} & \rrev{\brev{6.29}} & yes & 0.0075 & \brev{0.0046} & \brev{1.61} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.ces_Latn.{flores,multiblimp}
ell\_Grek & \rrev{\brev{0.0120}} & \rrev{\brev{0.0006}} & \rrev{\brev{19.32}} & yes & 0.0059 & \brev{0.0042} & \brev{1.43} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.ell_Grek.{flores,multiblimp}
tha\_Thai & \rrev{\brev{0.0188}} & \rrev{\brev{0.0013}} & \rrev{\brev{14.12}} & yes & -- & -- & -- & -- \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.tha_Thai.flores
fin\_Latn & \rrev{\brev{0.0209}} & \rrev{\brev{0.0050}} & \rrev{\brev{4.17}} & yes & 0.0092 & \brev{0.0052} & \brev{1.76} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.fin_Latn.{flores,multiblimp}
slk\_Latn & \rrev{\brev{0.0177}} & \rrev{\brev{0.0033}} & \rrev{\brev{5.39}} & yes & 0.0118 & \brev{0.0055} & \brev{2.16} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.slk_Latn.{flores,multiblimp}
bul\_Cyrl & \rrev{\brev{0.0070}} & \rrev{\brev{0.0020}} & \rrev{\brev{3.43}} & yes & 0.0107 & \brev{0.0088} & \brev{1.21} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.bul_Cyrl.{flores,multiblimp}
kor\_Hang & \rrev{\brev{0.0417}} & \rrev{\brev{0.0027}} & \rrev{\brev{15.70}} & yes & -- & -- & -- & -- \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.kor_Hang.flores
hrv\_Latn & \rrev{\brev{0.0191}} & \rrev{\brev{0.0046}} & \rrev{\brev{4.19}} & yes & -- & -- & -- & -- \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.hrv_Latn.flores
cat\_Latn & \rrev{\brev{0.0148}} & \rrev{\brev{0.0024}} & \rrev{\brev{6.20}} & yes & 0.0067 & \brev{0.0083} & \brev{0.80} & no \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.cat_Latn.{flores,multiblimp}
hin\_Deva & \rrev{\brev{0.0135}} & \rrev{\brev{0.0009}} & \rrev{\brev{14.35}} & yes & 0.0104 & \brev{0.0079} & \brev{1.32} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.hin_Deva.{flores,multiblimp}
heb\_Hebr & \rrev{\brev{0.0253}} & \rrev{\brev{0.0026}} & \rrev{\brev{9.64}} & yes & 0.0142 & \brev{0.0125} & \brev{1.13} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.heb_Hebr.{flores,multiblimp}
ben\_Beng & \rrev{\brev{0.0527}} & \rrev{\brev{0.0035}} & \rrev{\brev{15.03}} & yes & 0.0868 & \brev{0.0677} & \brev{1.28} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.ben_Beng.{flores,multiblimp}
tam\_Taml & \rrev{\brev{0.0312}} & \rrev{\brev{0.0021}} & \rrev{\brev{15.00}} & yes & 0.0231 & \brev{0.0062} & \brev{3.70} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.tam_Taml.{flores,multiblimp}
\bottomrule
\end{tabular}


==> crosslingual_tables/multiblimp.tex <==
\begin{tabular}{lcccc}
\toprule
\textbf{Intrinsic metric} & $\beta$ & SE$_{\text{m}}$ & SE$_{\text{cl}}$ & $p_{\text{adj}}^{\text{cl}}$ \\
\midrule
UTF-8 char split        & $-0.0066$ & $0.0006$ & $0.0014$ & $<10^{-5}$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_multiblimp.csv#utf8_char_split
Fertility               & $-0.0056$ & $0.0007$ & $0.0012$ & $<10^{-5}$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_multiblimp.csv#fertility
UTF-8 boundary crossing & $-0.0046$ & $0.0009$ & $0.0009$ & $<10^{-5}$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_multiblimp.csv#utf8_boundary_crossing
Trigram entropy         & $+0.0040$ & $0.0007$ & $0.0010$ & $<10^{-4}$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_multiblimp.csv#trigram_entropy
Bigram entropy          & $+0.0035$ & $0.0006$ & $0.0009$ & $<10^{-3}$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_multiblimp.csv#bigram_entropy
R\'enyi eff.\ ($\alpha{=}2$) & $+0.0031$ & $0.0006$ & $0.0007$ & $<10^{-4}$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_multiblimp.csv#renyi_2.0
Unigram entropy         & $+0.0029$ & $0.0007$ & $0.0009$ & $0.003$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_multiblimp.csv#unigram_entropy
Compression rate        & $+0.0029$ & $0.0008$ & $0.0009$ & $0.004$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_multiblimp.csv#compression_rate
Vocab utilization       & $-0.0002$ & $0.0011$ & $0.0010$ & $0.64$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_multiblimp.csv#vocab_utilization
\bottomrule
\end{tabular}


==> crosslingual_tables/optimizer.tex <==
\begin{tabular}{lllcl}
\toprule
\textbf{Group} & \textbf{Optimizer} & \textbf{Eff.\ LR} & \textbf{Betas} & \textbf{WD} \\
\midrule
Transformer matrices & Muon  & 0.0283{$^{*}$} & mom.\ schedule & 0.050$\to$0 \\
% prov: results/correlations/crosslingual_v2/optimizer_table_values.json#d24_optimizer.transformer_matrices.{effective_lr,weight_decay_peak,weight_decay_final}
Input embeddings     & AdamW & 0.2121 & (0.8, 0.995) & 0.001 \\
% prov: results/correlations/crosslingual_v2/optimizer_table_values.json#d24_optimizer.input_embeddings.{effective_lr,beta1,beta2,weight_decay}
Output projection    & AdamW & 0.0057 & (0.8, 0.96)  & 0.01 \\
% prov: results/correlations/crosslingual_v2/optimizer_table_values.json#d24_optimizer.output_projection.{effective_lr,beta1,beta2,weight_decay}
Value embeddings     & AdamW & 0.1061 & (0.8, 0.995) & 0.01 \\
% prov: results/correlations/crosslingual_v2/optimizer_table_values.json#d24_optimizer.value_embeddings.{effective_lr,beta1,beta2,weight_decay}
Residual scalars     & AdamW & 0.0071 & (0.8, 0.95)  & 0.05 \\
% prov: results/correlations/crosslingual_v2/optimizer_table_values.json#d24_optimizer.residual_scalars.{effective_lr,beta1,beta2,weight_decay}
Skip scalars         & AdamW & 0.707  & (0.96, 0.95) & 0.0 \\
% prov: results/correlations/crosslingual_v2/optimizer_table_values.json#d24_optimizer.skip_scalars.{effective_lr,beta1,beta2,weight_decay}
{Smear and backout parameters} & \rrev{AdamW} & \rrev{0.2} & \rrev{(0.8, 0.95)} & \rrev{0.0} \\
% prov: results/correlations/crosslingual_v2/optimizer_table_values.json#d24_optimizer.smear_backout_scalars.{effective_lr,beta1,beta2,weight_decay}
\bottomrule
\end{tabular}


==> crosslingual_tables/pretok.tex <==
\begin{tabular}{lccc}
\toprule
\textbf{Contrast (baseline $\to$ variant)} & \textbf{Mean $\Delta$} & \textbf{Langs.\ $>$ seed SD} & \textbf{above / below} \\
\midrule
GPT-4o $\to$ Claude        & $+0.0014$ & 17 / 31 & 8 / 9 \\
% prov: results/correlations/crosslingual_v2/perlang_controlled_deltas.json#pairs.pretok_gpt4o_vs_claude
GPT-4o $\to$ GPT-2         & $-0.0034$ & 24 / 31 & 5 / 19 \\
% prov: results/correlations/crosslingual_v2/perlang_controlled_deltas.json#pairs.pretok_gpt4o_vs_gpt2
GPT-4o $\to$ Punctuation   & $+0.0057$ & 17 / 31 & 15 / 2 \\
% prov: results/correlations/crosslingual_v2/perlang_controlled_deltas.json#pairs.pretok_gpt4o_vs_punct
GPT-4o $\to$ RightAlign    & $+0.0028$ & 15 / 31 & 12 / 3 \\
% prov: results/correlations/crosslingual_v2/perlang_controlled_deltas.json#pairs.pretok_gpt4o_vs_rightalign
GPT-4o $\to$ Whitespace    & $+0.0037$ & 16 / 31 & 14 / 2 \\
% prov: results/correlations/crosslingual_v2/perlang_controlled_deltas.json#pairs.pretok_gpt4o_vs_whitespace
\midrule
GPT-4 $\to$ Clean (PA-BPE) & $-0.0079$ & 21 / 31 & 1 / 20 \\
% prov: results/correlations/crosslingual_v2/perlang_controlled_deltas.json#pairs.pabpe_pretok_gpt4_vs_clean
PA-BPE base $\to$ hybrid-window & $-0.0090$ & 24 / 31 & 0 / 24 \\
% prov: results/correlations/crosslingual_v2/perlang_controlled_deltas.json#pairs.pabpe_merge_base_vs_hybridwindow
\bottomrule
\end{tabular}


==> crosslingual_tables/proxy-models.tex <==
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Layers} & \textbf{Width} & \textbf{Heads} & \textbf{Params} \\
\midrule
nanochat d8  & 8  & 512  & 4  & $0.22$B \\
% prov: results/correlations/crosslingual_v2/optimizer_table_values.json#proxy_models.d8.{n_layer,n_embd,n_head,params_total_billions}
nanochat d12 & 12 & 768  & 6  & $0.38$B \\
% prov: results/correlations/crosslingual_v2/optimizer_table_values.json#proxy_models.d12.{n_layer,n_embd,n_head,params_total_billions}
nanochat d16 & 16 & 1024 & 8  & $0.60$B \\
% prov: results/correlations/crosslingual_v2/optimizer_table_values.json#proxy_models.d16.{n_layer,n_embd,n_head,params_total_billions}
nanochat d24 (main) & 24 & 1536 & 12 & $1.27$B \\
% prov: results/correlations/crosslingual_v2/optimizer_table_values.json#proxy_models.d24.{n_layer,n_embd,n_head,params_total_billions}
\bottomrule
\end{tabular}


==> crosslingual_tables/proxy.tex <==
\begin{tabular}{lcc}
\toprule
\textbf{Ranking method} & \textbf{Val BPB} & \textbf{FLORES-tr.} \\
\midrule
Majority-class baseline                & \brev{$0.601$} & $0.565$ \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_pool9_summary.json#majority_class_floor
\midrule
All nine metrics (logistic ridge)      & \brev{$0.700$} & \rrev{$0.735$} \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_pool9_summary.json#targets.*.logistic_ridge_all_metrics
Best single metric, selected per fold  & \brev{$0.655$} & $0.668$ \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_pool9_summary.json#targets.*.best_single_per_fold
Bigram entropy (fixed)                 & \brev{$0.683$} & \rrev{$0.676$} \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_pool9_summary.json#targets.*.single_bigram_entropy
Trigram entropy (fixed)                & \brev{$0.639$} & $0.664$ \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_pool9_summary.json#targets.*.single_trigram_entropy
R\'enyi eff.\ ($\alpha{=}2$, fixed)    & \brev{$0.675$} & $0.653$ \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_pool9_summary.json#targets.*.single_renyi_2.0
Compression rate (fixed)               & \brev{$0.669$} & $0.657$ \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_pool9_summary.json#targets.*.single_compression_rate
\midrule
All nine metrics, per language ($278$ features) & \brev{$0.907$} & \rrev{$0.890$} \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_perlang_summary.json#targets.*.logistic_ridge_all_metrics
Best single feature, selected per fold        & \brev{$0.848$} & \rrev{$0.799$} \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_perlang_summary.json#targets.*.best_single_per_fold
Bigram entropy block (fixed)                & \brev{$0.910$} & \rrev{$0.909$} \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_perlang_summary.json#targets.*.single_bigram_entropy
Trigram entropy block (fixed)               & \brev{$0.879$} & \rrev{$0.865$} \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_perlang_summary.json#targets.*.single_trigram_entropy
R\'enyi eff.\ block ($\alpha{=}2$, fixed)   & \brev{$0.860$} & \rrev{$0.824$} \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_perlang_summary.json#targets.*.single_renyi_2.0
Compression rate block (fixed)              & \brev{$0.828$} & \rrev{$0.832$} \\
% prov: results/correlations/crosslingual_v2/loo_family_ranking_perlang_summary.json#targets.*.single_compression_rate
\midrule
Smaller model, d8 (val-BPB rank, $n{=}17$)  & \brev{$0.868$} & \rrev{$0.875$} \\
% prov: results/correlations/crosslingual_v2/cross_scale_transfer_v2.json#headline.{d8:val_bpb->val_bpb,d8:val_bpb->flores_trained_bpb}.agreement
Smaller model, d12 (val-BPB rank, $n{=}17$) & \brev{$0.846$} & \rrev{$0.853$} \\
% prov: results/correlations/crosslingual_v2/cross_scale_transfer_v2.json#headline.{d12:val_bpb->val_bpb,d12:val_bpb->flores_trained_bpb}.agreement
Smaller model, d16 (val-BPB rank, $n{=}17$) & \brev{$0.868$} & \rrev{$0.831$} \\
% prov: results/correlations/crosslingual_v2/cross_scale_transfer_v2.json#headline.{d16:val_bpb->val_bpb,d16:val_bpb->flores_trained_bpb}.agreement
\bottomrule
\end{tabular}


==> crosslingual_tables/repetition.tex <==
\begin{tabular}{lcc}
\toprule
& \textbf{Repeated} & \textbf{Fresh (single epoch)} \\
\midrule
Tamil    & \rrev{$+0.2674$} & \brev{\rrev{$+0.1386$}} \\
% prov: results/correlations/repetition_regime.json#exemplars.{repeated,fresh}.tam_Taml
Bengali  & \rrev{$+0.2616$} & \brev{\rrev{$+0.0997$}} \\
% prov: results/correlations/repetition_regime.json#exemplars.{repeated,fresh}.ben_Beng
Hebrew   & \rrev{$+0.0724$} & \brev{\rrev{$0.0059$}} \\
% prov: results/correlations/repetition_regime.json#exemplars.{repeated,fresh}.heb_Hebr
Korean   & \rrev{$+0.0468$} & \brev{\rrev{$-0.0087$}} \\
% prov: results/correlations/repetition_regime.json#exemplars.{repeated,fresh}.kor_Hang
\midrule
Mean (31 trained languages) & \rrev{$+0.0256$} & \brev{\rrev{$+0.0123$}} \\
% prov: results/correlations/repetition_regime.json#regime_difference.mean_dbpb.{repeated,fresh}
\bottomrule
\end{tabular}


==> crosslingual_tables/rq-map.tex <==
% ---- Candidate A: four accent-ruled cards ---------------------------------
% Uses only tcolorbox (already loaded; no extra tcolorbox library) and xcolor.
% No new packages, no preamble changes.
% "rqaccent" is defined here rather than in the preamble so the snippet is
% self-contained; the value is the paper's existing schemaccent (RGB 38,84,124),
% which is \definecolor'd in the body at the tokenizer-design figure and so is
% NOT in scope this early in the document.
\begingroup
\definecolor{rqaccent}{RGB}{38,84,124}
\footnotesize
\tcbset{rqcard/.style={%
  colback=rqaccent!5, colframe=rqaccent,
  boxrule=0pt, leftrule=1.6pt,
  sharp corners, boxsep=0pt,
  left=7pt, right=6pt, top=5pt, bottom=5.5pt,
  before skip=6pt, after skip=0pt, breakable=false}}
% run-in question: bold RQ tag, section badge, then the question in italic
\newcommand{\rqq}[3]{{\bfseries RQ#1}\hskip.5em
  {\color{rqaccent}\scriptsize\textsc{#2}}\hskip.8em
  {\itshape #3}\par}
% hairline, small-caps cue, then the answer in roman
\newcommand{\rqa}[1]{\vskip3.5pt
  {\color{rqaccent!40}\hrule height .4pt}\vskip4pt
  \noindent{\color{rqaccent}\scriptsize\textsc{answer}}\hskip.8em #1\par}
\begin{tcolorbox}[rqcard]
\rqq{1}{\cref{sec:magnitude}}{Holding the training setup fixed and varying only the tokenizer, how much does tokenizer choice change each language's BPB, MultiBLiMP accuracy, and XCOPA accuracy, relative to that language's seed-to-seed variation, and do tokenizers rank in the same order across languages?}
\rqa{Tokenizer choice changes every language's FLORES+ BPB, and MultiBLiMP accuracy for \brev{21} of the 24 covered languages, by more than that language's seed variation (XCOPA accuracies stay within a narrow band around chance), and the 54 tokenizers rank differently across languages: the mean rank agreement between two languages' orderings is Kendall $\tau = \rrev{0.418}$, and no single tokenizer ranks first for every language.}
% prov: results/correlations/crosslingual_v2/magnitude_table.json#summary.n_clears_floor.flores
% prov: results/correlations/crosslingual_v2/magnitude_table.json#summary.n_clears_floor.multiblimp
% prov: results/correlations/crosslingual_v2/battery_summary.json#kendall_overall_mean_offdiag_tau
% prov: results/correlations/crosslingual_v2/perlang_argmin.json#max_languages_won.n (supports the no-single-first clause, not printed)
\end{tcolorbox}
\begin{tcolorbox}[rqcard]
\rqq{2}{\cref{sec:sensitivity}}{Which language attributes (training-data share, inclusion in the tokenizer-training corpus, script, morphology) account for how sensitive a language is to tokenizer choice?}
\rqa{Languages with a smaller share of the language-model training data are more sensitive: the spread of a language's BPB across tokenizers falls as its share rises, and exclusion from tokenizer training raises a language's BPB more when its share is smaller; at 31 languages, resource level is not separable from writing system.}
\end{tcolorbox}
\begin{tcolorbox}[rqcard]
\rqq{3}{\cref{sec:design}}{Do individual design choices, including the reallocations proposed to benefit lower-resource languages (equal weighting, inverted weighting), change per-language outcomes by more than the seed variation, and in which direction for the languages whose share they raise?}
\rqa{\brev{18 of the 25 controlled design changes change at least one of the two aggregate outcomes by more than run-to-run variation}; the English-only restriction of the tokenizer-training data changes them most, and the two reallocations proposed to benefit lower-resource languages, equal and inverted weighting, raised BPB most for the languages whose share of the tokenizer-training data grew most (for the inverted allocation, a pattern specific to repeated training data); matching each language's training-token count removes only about a third of the largest increase.}
% prov: results/correlations/crosslingual_v2/floor_margins.json#threshold_scalars.n_controlled_pairs_clearing_on_at_least_one_outcome (printed as a rounded integer, not printed as a decimal)
% prov: results/correlations/crosslingual_v2/tokenmatch_readout.json#closure_fractions.repeated.tam_Taml (supports the about-a-third clause, not printed)
\end{tcolorbox}
\begin{tcolorbox}[rqcard]
\rqq{4}{\cref{sec:metrics}}{Which tokenizer properties computable without training account for a language's outcome, does the answer depend on the language's resource level, script, or morphology, and can a per-language ranking of tokenizers be predicted from the metrics alone, for tokenizer families not used to fit the prediction?}
\rqa{Within a language, tokenizers with higher entropy, R\'enyi efficiency, and compression rate have lower BPB\brev{ (for compression rate, only among models trained on the same number of tokens; after the adjustment for the number of training bytes, the unigram-entropy relationship is significant under two of our four estimates of the effect of training bytes, and the R\'enyi-efficiency relationship is significant under three of them)} and tokenizers with higher fertility and character-split rates have higher BPB, and which metric predicts BPB changes with resource tier, script, and morphology; measured per language, the nine metrics rank held-out tokenizer families at \rrev{$0.890$} to $0.907$ pairwise accuracy, against $0.700$ to $0.734$ for the same metrics as one value per tokenizer.}
% prov: results/correlations/crosslingual_v2/loo_family_ranking_perlang_summary.json#targets.val_bpb.logistic_ridge_all_metrics
% prov: results/correlations/crosslingual_v2/loo_family_ranking_perlang_summary.json#targets.flores_trained_bpb.logistic_ridge_all_metrics
% prov: results/correlations/crosslingual_v2/loo_family_ranking_pool9_summary.json#targets
\end{tcolorbox}
\endgroup


==> crosslingual_tables/seeded.tex <==
\begin{tabular}{lcc}
\toprule
\textbf{Contrast (baseline $\to$ variant)} & $\Delta$\textbf{BPB} & $p$ \\
\midrule
BPE $\to$ UnigramLM (GPT-4o)   & $+0.02929$ & $<10^{-35}$ \\
% prov: results/correlations/crosslingual_v2/perlang_controlled_deltas.json#seeded_contrasts.algo_bpe_vs_unigram_gpt4o_seeded
BPE $\to$ SuperBPE (GPT-4o)    & $+0.01275$ & $<10^{-17}$ \\
% prov: results/correlations/crosslingual_v2/perlang_controlled_deltas.json#seeded_contrasts.algo_bpe_vs_superbpe_gpt4o_seeded
GPT-4o $\to$ GPT-4o NFC        & \brev{$-0.00254$} & \brev{$0.16$} \\
% prov: results/correlations/crosslingual_v2/perlang_controlled_deltas.json#seeded_contrasts.nfc_gpt4o_seeded
GPT-4o $\to$ Claude (pretok)   & $+0.00044$ & $0.71$ \\
% prov: results/correlations/crosslingual_v2/perlang_controlled_deltas.json#seeded_contrasts.pretok_gpt4o_vs_claude_seeded
\bottomrule
\end{tabular}


==> crosslingual_tables/select.tex <==
\begin{tabular}{llrrrr}
\toprule
& \textbf{Contrast (baseline $\to$ variant)} & $\Delta$\textbf{FLORES} & ratio & $\Delta$\textbf{Val} & ratio \\
\midrule
\multirow{6}{*}{\rotatebox{90}{Data}}
& Balanced $\to$ English-only (GPT-4o)$^{a}$   & \rrev{$\mathbf{+0.0386}$} & \rrev{$32.69$} & \brev{$\mathbf{+0.0332}$} & \brev{$81.73$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#data_gpt4o_balanced_vs_english_fullbyte; results/correlations/crosslingual_v2/floor_margins.json#pairs.data_gpt4o_balanced_vs_english_fullbyte.{flores_trained_margin_mean_floor,val_margin}
& Balanced $\to$ English-only (Claude)$^{b}$   & \rrev{$\mathbf{+0.0307}$} & \rrev{$26.06$} & \brev{$\mathbf{+0.0248}$} & \brev{$61.00$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#data_claude_balanced_vs_english; results/correlations/crosslingual_v2/floor_margins.json#pairs.data_claude_balanced_vs_english.{flores_trained_margin_mean_floor,val_margin}
& Balanced $\to$ English-only (Punct)$^{b}$    & \rrev{$\mathbf{+0.0238}$} & \rrev{$20.18$} & \brev{$\mathbf{+0.0254}$} & \brev{$62.41$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#data_punct_balanced_vs_english; results/correlations/crosslingual_v2/floor_margins.json#pairs.data_punct_balanced_vs_english.{flores_trained_margin_mean_floor,val_margin}
& Balanced $\to$ Code-heavy (GPT-4o)           & \rrev{$\mathbf{+0.0189}$} & \rrev{$16.06$} & \brev{$\mathbf{+0.0153}$} & \brev{$37.56$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#data_gpt4o_balanced_vs_code; results/correlations/crosslingual_v2/floor_margins.json#pairs.data_gpt4o_balanced_vs_code.{flores_trained_margin_mean_floor,val_margin}
& Balanced $\to$ High-resource (GPT-4o)        & \rrev{$\mathbf{+0.0202}$} & \rrev{$17.09$} & \brev{$+0.00025$} & \brev{$0.62$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#data_gpt4o_balanced_vs_highres; results/correlations/crosslingual_v2/floor_margins.json#pairs.data_gpt4o_balanced_vs_highres.{flores_trained_margin_mean_floor,val_margin}
& Balanced $\to$ High+mid (GPT-4o)             & \rrev{$\mathbf{+0.0121}$} & \rrev{$10.29$} & \brev{$+0.00059$} & \brev{$1.45$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#data_gpt4o_balanced_vs_highmid; results/correlations/crosslingual_v2/floor_margins.json#pairs.data_gpt4o_balanced_vs_highmid.{flores_trained_margin_mean_floor,val_margin}
\midrule
\multirow{6}{*}{\rotatebox{90}{Algorithm}}
& BPE $\to$ UnigramLM (GPT-4o)                 & $\mathbf{+0.0323}$ & \rrev{$27.41$} & \brev{$\mathbf{+0.0199}$} & \brev{$48.92$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#algo_bpe_vs_unigram_gpt4o; results/correlations/crosslingual_v2/floor_margins.json#pairs.algo_bpe_vs_unigram_gpt4o.{flores_trained_margin_mean_floor,val_margin}
& BPE $\to$ UnigramLM (Claude)                 & \rrev{$\mathbf{+0.0285}$} & \rrev{$24.19$} & \brev{$\mathbf{+0.0198}$} & \brev{$48.81$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#algo_bpe_vs_unigram_claude; results/correlations/crosslingual_v2/floor_margins.json#pairs.algo_bpe_vs_unigram_claude.{flores_trained_margin_mean_floor,val_margin}
& BPE $\to$ UnigramLM (RightAlign)             & \rrev{$\mathbf{+0.0293}$} & \rrev{$24.86$} & \brev{$\mathbf{+0.0192}$} & \brev{$47.32$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#algo_bpe_vs_unigram_rightalign; results/correlations/crosslingual_v2/floor_margins.json#pairs.algo_bpe_vs_unigram_rightalign.{flores_trained_margin_mean_floor,val_margin}
& BPE $\to$ SuperBPE (GPT-4o)                  & \rrev{$\mathbf{+0.0130}$} & \rrev{$11.02$} & $\mathbf{+0.0105}$ & \brev{$25.94$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#superbpe_gpt4o_base_vs_superword; results/correlations/crosslingual_v2/floor_margins.json#pairs.superbpe_gpt4o_base_vs_superword.{flores_trained_margin_mean_floor,val_margin}
& PA-BPE $\to$ SuperBPE+PA-BPE (GPT-4o)%\brev{$^{c}$} 
& \rrev{$-0.0025$} & \rrev{$2.11$} & \brev{$\mathbf{+0.0035}$} & \brev{$8.51$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#superbpe_pabpe_base_vs_superword; results/correlations/crosslingual_v2/floor_margins.json#pairs.superbpe_pabpe_base_vs_superword.{flores_trained_margin_mean_floor,val_margin}
& BPE $\to$ PA-BPE (Clean, NFC)                & \rrev{$\mathbf{+0.0200}$} & \rrev{$16.95$} & \brev{$\mathbf{+0.0086}$} & \brev{$21.11$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#trainer_clean_bpe_vs_pabpe; results/correlations/crosslingual_v2/floor_margins.json#pairs.trainer_clean_bpe_vs_pabpe.{flores_trained_margin_mean_floor,val_margin}
\midrule
\multirow{6}{*}{\rotatebox{90}{Pretokenizer}}
& GPT-4o $\to$ Claude                          & \brev{$+0.0014$} & \rrev{$1.18$} & $\mathbf{+0.0024}$ & \brev{$5.89$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#pretok_gpt4o_vs_claude; results/correlations/crosslingual_v2/floor_margins.json#pairs.pretok_gpt4o_vs_claude.{flores_trained_margin_mean_floor,val_margin}
& GPT-4o $\to$ GPT-2                           & \rrev{\brev{$-0.0018$}} & \rrev{$1.55$} & \brev{$-0.00033$} & \brev{$0.81$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#pretok_gpt4o_vs_gpt2; results/correlations/crosslingual_v2/floor_margins.json#pairs.pretok_gpt4o_vs_gpt2.{flores_trained_margin_mean_floor,val_margin}
& GPT-4o $\to$ Punctuation                     & \rrev{$\mathbf{+0.0048}$} & \rrev{$4.07$} & $\mathbf{+0.0054}$ & \brev{$13.27$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#pretok_gpt4o_vs_punct; results/correlations/crosslingual_v2/floor_margins.json#pairs.pretok_gpt4o_vs_punct.{flores_trained_margin_mean_floor,val_margin}
& GPT-4o $\to$ RightAlign                      & \rrev{\brev{$+0.0030$}} & \rrev{$2.52$} & \brev{$+0.00066$} & \brev{$1.62$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#pretok_gpt4o_vs_rightalign; results/correlations/crosslingual_v2/floor_margins.json#pairs.pretok_gpt4o_vs_rightalign.{flores_trained_margin_mean_floor,val_margin}
& GPT-4o $\to$ Whitespace                      & \rrev{$\mathbf{+0.0049}$} & \rrev{$4.19$} & \brev{$\mathbf{+0.0078}$} & \brev{$19.23$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#pretok_gpt4o_vs_whitespace; results/correlations/crosslingual_v2/floor_margins.json#pairs.pretok_gpt4o_vs_whitespace.{flores_trained_margin_mean_floor,val_margin}
& GPT-4o $\to$ Clean (PA-BPE)                   & \rrev{$\mathbf{-0.0070}$} & \rrev{$5.95$} & \brev{$\mathbf{-0.0019}$} & \brev{$4.75$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#pabpe_pretok_gpt4_vs_clean; results/correlations/crosslingual_v2/floor_margins.json#pairs.pabpe_pretok_gpt4_vs_clean.{flores_trained_margin_mean_floor,val_margin}
\midrule
\multirow{3}{*}{\rotatebox{90}{NFC}}
& GPT-4o $\to$ GPT-4o NFC                      & \rrev{\brev{$-0.0019$}} & \rrev{$1.65$} & $+0.00022$ & $0.55$ \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#nfc_gpt4o; results/correlations/crosslingual_v2/floor_margins.json#pairs.nfc_gpt4o.{flores_trained_margin_mean_floor,val_margin}
& Claude $\to$ Claude NFC                      & \rrev{\brev{$-0.0036$}} & \rrev{$3.08$} & \brev{$-0.00033$} & \brev{$0.81$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#nfc_claude; results/correlations/crosslingual_v2/floor_margins.json#pairs.nfc_claude.{flores_trained_margin_mean_floor,val_margin}
& RightAlign $\to$ RightAlign NFC              & \rrev{\brev{$-0.0038$}} & \rrev{$3.22$} & \brev{$+0.00002$} & \brev{$0.05$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#nfc_rightalign; results/correlations/crosslingual_v2/floor_margins.json#pairs.nfc_rightalign.{flores_trained_margin_mean_floor,val_margin}
\midrule
\multirow{4}{*}{\rotatebox{90}{Presets}}
& UnigramLM default $\to$ tuned (GPT-4o)       & \rrev{$-0.0004$} & \rrev{$0.33$} & \brev{$-0.00002$} & \brev{$0.06$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#unigram_tuning_gpt4o; results/correlations/crosslingual_v2/floor_margins.json#pairs.unigram_tuning_gpt4o.{flores_trained_margin_mean_floor,val_margin}
& PA-BPE base $\to$ hybrid-window (GPT-4o)      & \rrev{$\mathbf{-0.0084}$} & \rrev{$7.11$} & \brev{$\mathbf{-0.0065}$} & \brev{$15.88$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#pabpe_merge_base_vs_hybridwindow; results/correlations/crosslingual_v2/floor_margins.json#pairs.pabpe_merge_base_vs_hybridwindow.{flores_trained_margin_mean_floor,val_margin}
& SuperBPE+PA-BPE t90k $\to$ t64k              & \rrev{$-0.0004$} & \rrev{$0.37$} & \brev{$-0.00008$} & \brev{$0.20$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#superbpe_budget_t90k_vs_t64k; results/correlations/crosslingual_v2/floor_margins.json#pairs.superbpe_budget_t90k_vs_t64k.{flores_trained_margin_mean_floor,val_margin}
& SuperBPE Clean C2 $\to$ C3                   & \rrev{$\mathbf{+0.0044}$} & \rrev{$3.75$} & \brev{$\mathbf{+0.0012}$} & \brev{$2.88$} \\
% prov: results/correlations/crosslingual_v2/controlled_comparisons_v2.json#superbpe_regex_c2_vs_c3; results/correlations/crosslingual_v2/floor_margins.json#pairs.superbpe_regex_c2_vs_c3.{flores_trained_margin_mean_floor,val_margin}
\bottomrule
\end{tabular}


==> crosslingual_tables/share-gain-loss.tex <==
\begin{tabular}{llll}
\toprule
& \textbf{Variant} & \textbf{Largest gains (pp)} & \textbf{Largest losses (pp)} \\
\midrule
\multirow{5}{*}{\rotatebox{90}{Equal}}
& Equal (GPT-4o)$^{c}$ & \brev{eng $+0.35$, tha $+0.02$, ell $+0.02$} & \brev{rus $-0.82$} \\
% prov: results/correlations/crosslingual_v2/share_gain_loss.json#arms.allmulti-equal-bpe.{top_gainers,top_losers}
& Equal (Claude) & \brev{eng $+0.33$, tha $+0.02$, ell $+0.02$} & \brev{rus $-0.76$, spa $-0.01$, cmn $-0.01$} \\
% prov: results/correlations/crosslingual_v2/share_gain_loss.json#arms.claude-allmulti-equal-bpe.{top_gainers,top_losers}
& Equal (GPT-4o, NFC) & \brev{eng $+0.35$, tha $+0.02$, ell $+0.02$} & \brev{rus $-0.82$} \\
% prov: results/correlations/crosslingual_v2/share_gain_loss.json#arms.gpt4o-allmulti-equal-nfc-bpe.{top_gainers,top_losers}
& Equal, no repeat (GPT-4o)$^{c}$ & \brev{eng $+0.35$, tha $+0.02$, ell $+0.02$} & \brev{rus $-0.82$} \\
% prov: results/correlations/crosslingual_v2/share_gain_loss.json#arms.gpt4o-allmulti-equal-norepeat-bpe.{top_gainers,top_losers}
& Equal (Punctuation) & \brev{eng $+0.30$, ell $+0.02$, tha $+0.02$} & \brev{rus $-0.68$, cmn $-0.01$} \\
% prov: results/correlations/crosslingual_v2/share_gain_loss.json#arms.punct-allmulti-equal-bpe.{top_gainers,top_losers}
\midrule
\multirow{4}{*}{\rotatebox{90}{Inversion}}
& Inverted & \brev{eng $+0.49$, tha $+0.03$, ces $+0.02$} & \brev{rus $-1.61$, ind $-0.03$, cmn $-0.03$} \\
% prov: results/correlations/crosslingual_v2/share_gain_loss.json#arms.gpt4o-invert-full-bpe.{top_gainers,top_losers}
& No English & \brev{rus $+0.25$, fra $+0.02$, deu $+0.02$} & \brev{eng $-0.55$} \\
% prov: results/correlations/crosslingual_v2/share_gain_loss.json#arms.gpt4o-no-english-bpe.{top_gainers,top_losers}
& Permutation A & \brev{eng $+0.17$, arb $+0.05$, ell $+0.05$} & \brev{rus $-0.99$, spa $-0.03$, fra $-0.03$} \\
% prov: results/correlations/crosslingual_v2/share_gain_loss.json#arms.gpt4o-perm-a-bpe.{top_gainers,top_losers}
& Permutation B & \brev{eng $+0.38$, spa $+0.03$, tha $+0.02$} & \brev{rus $-1.29$, ell $-0.01$, ind $-0.01$} \\
% prov: results/correlations/crosslingual_v2/share_gain_loss.json#arms.gpt4o-perm-b-bpe.{top_gainers,top_losers}
\bottomrule
\end{tabular}


==> crosslingual_tables/tier.tex <==
\begin{tabular}{lccc}
\toprule
\textbf{Intrinsic metric} & \textbf{High} & \textbf{Mid} & \textbf{Low} \\
\midrule
Trigram entropy              & \rrev{$\mathbf{-0.0111}$} & \rrev{$\mathbf{-0.0084}$} & \rrev{$\mathbf{-0.0128}$} \\ 
% prov: results/correlations/crosslingual_v2/cross_lingual_A1_tier_betas.csv#trigram_entropy; clustered_moderation.csv#[block=tier][term=trigram_entropy|{high,mid,low}]
UTF-8 char split             & \rrev{$\mathbf{+0.0215}$} & \rrev{$\mathbf{+0.0074}$} & \rrev{$\mathbf{+0.0119}$} \\ 
% prov: results/correlations/crosslingual_v2/cross_lingual_A1_tier_betas.csv#utf8_char_split; clustered_moderation.csv#[block=tier][term=utf8_char_split|{high,mid,low}]
Vocab utilization            & \rrev{$-0.0052$} & \rrev{$+0.0012$} & \rrev{$\mathbf{+0.0112}$} \\ 
% prov: results/correlations/crosslingual_v2/cross_lingual_A1_tier_betas.csv#vocab_utilization; clustered_moderation.csv#[block=tier][term=vocab_utilization|{high,mid,low}]
R\'enyi eff.\ ($\alpha{=}2$) & \rrev{$-0.0002$} & \rrev{$\mathbf{-0.0065}$} & \rrev{$\mathbf{-0.0105}$} \\ 
% prov: results/correlations/crosslingual_v2/cross_lingual_A1_tier_betas.csv#renyi_2.0; clustered_moderation.csv#[block=tier][term=renyi_2.0|{high,mid,low}]
Fertility                    & \rrev{$\mathbf{+0.0539}$} & \rrev{$\mathbf{+0.0070}$} & \rrev{$\mathbf{+0.0099}$} \\ 
% prov: results/correlations/crosslingual_v2/cross_lingual_A1_tier_betas.csv#fertility; clustered_moderation.csv#[block=tier][term=fertility|{high,mid,low}]
Bigram entropy               & \rrev{$-0.0060$} & \rrev{$\mathbf{-0.0077}$} & \rrev{$\mathbf{-0.0094}$} \\ 
% prov: results/correlations/crosslingual_v2/cross_lingual_A1_tier_betas.csv#bigram_entropy; clustered_moderation.csv#[block=tier][term=bigram_entropy|{high,mid,low}]
Unigram entropy              & \rrev{$-0.0062$} & \rrev{$\mathbf{-0.0059}$} & \rrev{$-0.0059$} \\ 
% prov: results/correlations/crosslingual_v2/cross_lingual_A1_tier_betas.csv#unigram_entropy; clustered_moderation.csv#[block=tier][term=unigram_entropy|{high,mid,low}]
Compression rate             & \rrev{$-0.0103$} & \rrev{$\mathbf{-0.0063}$} & \rrev{$-0.0043$} \\ 
% prov: results/correlations/crosslingual_v2/cross_lingual_A1_tier_betas.csv#compression_rate; clustered_moderation.csv#[block=tier][term=compression_rate|{high,mid,low}]
UTF-8 boundary crossing      & \rrev{$\mathbf{+0.0101}$} & \rrev{$\mathbf{+0.0028}$} & \rrev{$+0.0028$} \\ 
% prov: results/correlations/crosslingual_v2/cross_lingual_A1_tier_betas.csv#utf8_boundary_crossing; clustered_moderation.csv#[block=tier][term=utf8_boundary_crossing|{high,mid,low}]
\bottomrule
\end{tabular}


==> crosslingual_tables/within-budget.tex <==
\begin{tabular}{lrrrrr}
\toprule
& \multicolumn{1}{c}{\textbf{unadjusted}} & \multicolumn{4}{c}{\textbf{estimate of $\beta$ used in the adjustment}} \\
\cmidrule(lr){3-6}
\textbf{Metric} & & $-0.0186$ & $-0.0257$ & \brev{$-0.0365$} & $-0.0397$ \\
\midrule
Fertility & \rrev{$+0.0154^{*}$} & \brev{\rrev{$+0.0154^{*}$}} & \brev{\rrev{$+0.0147^{*}$}} & \brev{\rrev{$+0.0135^{*}$}} & \brev{\rrev{$+0.0135^{*}$}} \\
% prov: results/correlations/crosslingual_v2/budget_adjusted_panel.json#tab_within_all_metrics_refit.results.{baseline_n51_unadjusted,r7_superbpe_point_advisory,continue_point,r7_unigram_point_advisory,fresh160_mean_advisory}.per_metric.fertility.coefficient_fe
UTF-8 char split & \rrev{$+0.0113^{*}$} & \rrev{$+0.0113^{*}$} & \brev{$+0.0108^{*}$} & \rrev{$+0.0099^{*}$} & \rrev{$+0.0099^{*}$} \\
% prov: results/correlations/crosslingual_v2/budget_adjusted_panel.json#tab_within_all_metrics_refit.results.{baseline_n51_unadjusted,r7_superbpe_point_advisory,continue_point,r7_unigram_point_advisory,fresh160_mean_advisory}.per_metric.utf8_char_split.coefficient_fe
Trigram entropy & \rrev{$-0.0110^{*}$} & \brev{\rrev{$-0.0109^{*}$}} & \brev{\rrev{$-0.0095^{*}$}} & \brev{\rrev{$-0.0070^{*}$}} & \brev{\rrev{$-0.0072^{*}$}} \\
% prov: results/correlations/crosslingual_v2/budget_adjusted_panel.json#tab_within_all_metrics_refit.results.{baseline_n51_unadjusted,r7_superbpe_point_advisory,continue_point,r7_unigram_point_advisory,fresh160_mean_advisory}.per_metric.trigram_entropy.coefficient_fe
Bigram entropy & $-0.0083^{*}$ & \brev{\rrev{$-0.0082^{*}$}} & \brev{\rrev{$-0.0067^{*}$}} & \brev{\rrev{$-0.0039^{*}$}} & \brev{$-0.0041^{*}$} \\
% prov: results/correlations/crosslingual_v2/budget_adjusted_panel.json#tab_within_all_metrics_refit.results.{baseline_n51_unadjusted,r7_superbpe_point_advisory,continue_point,r7_unigram_point_advisory,fresh160_mean_advisory}.per_metric.bigram_entropy.coefficient_fe
Compression rate & \rrev{$-0.0071^{*}$} & \brev{\rrev{$-0.0070^{*}$}} & \brev{\rrev{$-0.0055$}} & \brev{\rrev{$-0.0029$}} & \brev{\rrev{$-0.0031$}} \\
% prov: results/correlations/crosslingual_v2/budget_adjusted_panel.json#tab_within_all_metrics_refit.results.{baseline_n51_unadjusted,r7_superbpe_point_advisory,continue_point,r7_unigram_point_advisory,fresh160_mean_advisory}.per_metric.compression_rate.coefficient_fe
R\'enyi eff.\ ($\alpha{=}2$) & \rrev{$-0.0071^{*}$} & \brev{\rrev{$-0.0070^{*}$}} & \brev{\rrev{$-0.0055^{*}$}} & \brev{\rrev{$-0.0027^{*}$}} & \brev{\rrev{$-0.0029$}} \\
% prov: results/correlations/crosslingual_v2/budget_adjusted_panel.json#tab_within_all_metrics_refit.results.{baseline_n51_unadjusted,r7_superbpe_point_advisory,continue_point,r7_unigram_point_advisory,fresh160_mean_advisory}.per_metric.renyi_2.0.coefficient_fe
Unigram entropy & \rrev{$-0.0065^{*}$} & \brev{\rrev{$-0.0064^{*}$}} & \brev{\rrev{$-0.0050^{*}$}} & \brev{\rrev{$-0.0026$}} & \brev{\rrev{$-0.0028$}} \\
% prov: results/correlations/crosslingual_v2/budget_adjusted_panel.json#tab_within_all_metrics_refit.results.{baseline_n51_unadjusted,r7_superbpe_point_advisory,continue_point,r7_unigram_point_advisory,fresh160_mean_advisory}.per_metric.unigram_entropy.coefficient_fe
UTF-8 boundary crossing & \rrev{$+0.0025^{*}$} & \rrev{$+0.0025^{*}$} & \rrev{$+0.0023^{*}$} & \brev{\rrev{$+0.0020^{*}$}} & \rrev{$+0.0020^{*}$} \\
% prov: results/correlations/crosslingual_v2/budget_adjusted_panel.json#tab_within_all_metrics_refit.results.{baseline_n51_unadjusted,r7_superbpe_point_advisory,continue_point,r7_unigram_point_advisory,fresh160_mean_advisory}.per_metric.utf8_boundary_crossing.coefficient_fe
Vocab.\ utilization & \rrev{$+0.0011$} & \brev{\rrev{$+0.0012$}} & \brev{\rrev{$+0.0022$}} & \brev{\rrev{$+0.0041$}} & \brev{\rrev{$+0.0040$}} \\
% prov: results/correlations/crosslingual_v2/budget_adjusted_panel.json#tab_within_all_metrics_refit.results.{baseline_n51_unadjusted,r7_superbpe_point_advisory,continue_point,r7_unigram_point_advisory,fresh160_mean_advisory}.per_metric.vocab_utilization.coefficient_fe
\bottomrule
\end{tabular}


==> crosslingual_tables/within-fw2.tex <==
\begin{tabular}{lccccc}
\toprule
\textbf{Intrinsic metric} & $\beta$ & SE$_{\text{m}}$ & SE$_{\text{cl}}$ & $p_{\text{adj}}^{\text{cl}}$ & $R^2$ \\
\midrule
Fertility               & $+0.0322$ & $0.0014$ & $0.0022$ & $<10^{-47}$ & $0.244$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_fw2.csv#fertility; cross_lingual_C_variance_fw2.csv#fertility.within_lang_r2
Trigram entropy         & $-0.0168$ & $0.0005$ & $0.0016$ & $<10^{-26}$ & $0.458$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_fw2.csv#trigram_entropy; cross_lingual_C_variance_fw2.csv#trigram_entropy.within_lang_r2
Unigram entropy         & $-0.0151$ & $0.0005$ & $0.0020$ & $<10^{-13}$ & $0.329$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_fw2.csv#unigram_entropy; cross_lingual_C_variance_fw2.csv#unigram_entropy.within_lang_r2
Compression rate        & $-0.0151$ & $0.0007$ & $0.0027$ & $<10^{-7}$  & $0.240$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_fw2.csv#compression_rate; cross_lingual_C_variance_fw2.csv#compression_rate.within_lang_r2
Bigram entropy          & $-0.0145$ & $0.0004$ & $0.0017$ & $<10^{-17}$ & $0.396$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_fw2.csv#bigram_entropy; cross_lingual_C_variance_fw2.csv#bigram_entropy.within_lang_r2
UTF-8 char split        & $+0.0140$ & $0.0005$ & $0.0008$ & $<10^{-71}$ & $0.344$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_fw2.csv#utf8_char_split; cross_lingual_C_variance_fw2.csv#utf8_char_split.within_lang_r2
R\'enyi eff.\ ($\alpha{=}2$) & $-0.0121$ & $0.0005$ & $0.0015$ & $<10^{-14}$ & $0.298$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_fw2.csv#renyi_2.0; cross_lingual_C_variance_fw2.csv#renyi_2.0.within_lang_r2
Vocab utilization       & $-0.0076$ & $0.0010$ & $0.0008$ & $<10^{-18}$ & $0.035$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_fw2.csv#vocab_utilization; cross_lingual_C_variance_fw2.csv#vocab_utilization.within_lang_r2
UTF-8 boundary crossing & $+0.0022$ & $0.0007$ & $0.0010$ & $0.026$     & $0.005$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_fw2.csv#utf8_boundary_crossing; cross_lingual_C_variance_fw2.csv#utf8_boundary_crossing.within_lang_r2
\bottomrule
\end{tabular}


==> crosslingual_tables/within.tex <==
\begin{tabular}{lccccc}
\toprule
\textbf{Intrinsic metric} & $\beta$ & SE$_{\text{m}}$ & SE$_{\text{cl}}$ & $p_{\text{adj}}^{\text{cl}}$ & $R^2$ \\
\midrule
Fertility               & \rrev{$+0.0156$} & \rrev{$0.0013$} & \rrev{$0.0027$} & \rrev{$<10^{-7}$} & \rrev{$0.082$} \\ 
% prov: results/correlations/crosslingual_v2/mixed_effects.csv#fertility; cross_lingual_C_variance.csv#fertility.within_lang_r2
UTF-8 char split        & \rrev{$+0.0113$} & \rrev{$0.0005$} & \rrev{$0.0012$} & $<10^{-16}$ & \rrev{$0.214$} \\ 
% prov: results/correlations/crosslingual_v2/mixed_effects.csv#utf8_char_split; cross_lingual_C_variance.csv#utf8_char_split.within_lang_r2
Trigram entropy         & \rrev{$-0.0112$} & \rrev{$0.0006$} & \rrev{$0.0015$} & $<10^{-13}$ & \rrev{$0.170$} \\ 
% prov: results/correlations/crosslingual_v2/mixed_effects.csv#trigram_entropy; cross_lingual_C_variance.csv#trigram_entropy.within_lang_r2
Bigram entropy          & \rrev{$-0.0083$} & $0.0006$ & \rrev{$0.0017$} & \rrev{$<10^{-5}$} & \rrev{$0.120$} \\ 
% prov: results/correlations/crosslingual_v2/mixed_effects.csv#bigram_entropy; cross_lingual_C_variance.csv#bigram_entropy.within_lang_r2
Compression rate        & \rrev{$-0.0072$} & \rrev{$0.0007$} & \rrev{$0.0024$} & $0.003$     & \rrev{$0.057$} \\ 
% prov: results/correlations/crosslingual_v2/mixed_effects.csv#compression_rate; cross_lingual_C_variance.csv#compression_rate.within_lang_r2
R\'enyi eff.\ ($\alpha{=}2$) & \rrev{$-0.0070$} & \rrev{$0.0005$} & \rrev{$0.0015$} & $<10^{-5}$ & \rrev{$0.093$} \\ 
% prov: results/correlations/crosslingual_v2/mixed_effects.csv#renyi_2.0; cross_lingual_C_variance.csv#renyi_2.0.within_lang_r2
Unigram entropy         & \rrev{$-0.0064$} & \rrev{$0.0006$} & $0.0021$ & \rrev{$0.003$} & \rrev{$0.056$} \\ 
% prov: results/correlations/crosslingual_v2/mixed_effects.csv#unigram_entropy; cross_lingual_C_variance.csv#unigram_entropy.within_lang_r2
UTF-8 boundary crossing & \rrev{$+0.0028$} & $0.0008$ & $0.0008$ & \rrev{$<10^{-3}$} & \rrev{$0.007$} \\ 
% prov: results/correlations/crosslingual_v2/mixed_effects.csv#utf8_boundary_crossing; cross_lingual_C_variance.csv#utf8_boundary_crossing.within_lang_r2
Vocab utilization       & \rrev{$+0.0013$} & $0.0010$ & \rrev{$0.0030$} & \rrev{$0.67$} & $0.000$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects.csv#vocab_utilization; cross_lingual_C_variance.csv#vocab_utilization.within_lang_r2
\bottomrule
\end{tabular}


==> crosslingual_tables/xcopa-magnitude.tex <==
\begin{tabular}{lrrrc}
\toprule
\textbf{Language} & spread & seed SD & ratio & clears \\
\midrule
cmn\_Hans & 0.0155 & \brev{0.0150} & \brev{1.03} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.cmn_Hans.xcopa
ita\_Latn & 0.0145 & \brev{0.0087} & \brev{1.66} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.ita_Latn.xcopa
tur\_Latn & 0.0184 & \brev{0.0185} & \brev{1.00} & no \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.tur_Latn.xcopa
ind\_Latn & 0.0155 & \brev{0.0113} & \brev{1.38} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.ind_Latn.xcopa
vie\_Latn & 0.0143 & \brev{0.0104} & \brev{1.38} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.vie_Latn.xcopa
tha\_Thai & 0.0159 & \brev{0.0167} & \brev{0.95} & no \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.tha_Thai.xcopa
tam\_Taml & 0.0154 & \brev{0.0116} & \brev{1.33} & yes \\
% prov: results/correlations/crosslingual_v2/magnitude_table.json#rows.tam_Taml.xcopa
\bottomrule
\end{tabular}


==> crosslingual_tables/xnli.tex <==
\begin{tabular}{lcccc}
\toprule
\textbf{Intrinsic metric} & $\beta$ & SE$_{\text{m}}$ & SE$_{\text{cl}}$ & $p_{\text{adj}}^{\text{cl}}$ \\
\midrule
Fertility               & $-0.0043$ & $0.0012$ & $0.0009$ & $<10^{-5}$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_xnli.csv#fertility
Trigram entropy         & $+0.0042$ & $0.0008$ & $0.0010$ & $<10^{-4}$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_xnli.csv#trigram_entropy
UTF-8 char split        & $-0.0030$ & $0.0006$ & $0.0007$ & $<10^{-4}$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_xnli.csv#utf8_char_split
Compression rate        & $+0.0023$ & $0.0008$ & $0.0011$ & $0.07$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_xnli.csv#compression_rate
UTF-8 boundary crossing & $-0.0020$ & $0.0006$ & $0.0004$ & $<10^{-5}$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_xnli.csv#utf8_boundary_crossing
Unigram entropy         & $+0.0019$ & $0.0007$ & $0.0010$ & $0.08$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_xnli.csv#unigram_entropy
Bigram entropy          & $+0.0019$ & $0.0006$ & $0.0010$ & $0.07$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_xnli.csv#bigram_entropy
Vocab utilization       & $+0.0010$ & $0.0010$ & $0.0011$ & $0.52$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_xnli.csv#vocab_utilization
R\'enyi eff.\ ($\alpha{=}2$) & $+0.0006$ & $0.0006$ & $0.0011$ & $0.58$ \\
% prov: results/correlations/crosslingual_v2/mixed_effects_xnli.csv#renyi_2.0
\bottomrule
\end{tabular}
